Multi-Objective Coordination Graphs for the Expected Scalarised Returns with Generative Flow Models

Many real-world problems contain multiple objectives and agents, where a trade-off exists between objectives. Key to solving such problems is to exploit sparse dependency structures that exist between agents. For example, in wind farm control a trade-off exists between maximising power and minimising stress on the systems components. Dependencies between turbines arise due to the wake effect. We model such sparse dependencies between agents as a multi-objective coordination graph (MO-CoG). In multi-objective reinforcement learning a utility function is typically used to model a users preferences over objectives, which may be unknown a priori. In such settings a set of optimal policies must be computed. Which policies are optimal depends on which optimality criterion applies. If the utility function of a user is derived from multiple executions of a policy, the scalarised expected returns (SER) must be optimised. If the utility of a user is derived from a single execution of a policy, the expected scalarised returns (ESR) criterion must be optimised. For example, wind farms are subjected to constraints and regulations that must be adhered to at all times, therefore the ESR criterion must be optimised. For MO-CoGs, the state-of-the-art algorithms can only compute a set of optimal policies for the SER criterion, leaving the ESR criterion understudied. To compute a set of optimal polices under the ESR criterion, also known as the ESR set, distributions over the returns must be maintained. Therefore, to compute a set of optimal policies under the ESR criterion for MO-CoGs, we present a novel distributional multi-objective variable elimination (DMOVE) algorithm. We evaluate DMOVE in realistic wind farm simulations. Given the returns in real-world wind farm settings are continuous, we utilise a model known as real-NVP to learn the continuous return distributions to calculate the ESR set.

==> plotting.tex <==
\begin{tikzpicture}
\pgfplotsset{
      scale only axis,
      %date coordinates in=x,
      %xticklabel=\day/\month,
      height=3cm,
      every axis label={font=5}
    }
    \begin{groupplot}[
    group style={
            % set how the plots should be organized
            group size=4 by 5,
            % only show ticklabels and axis labels on the bottom
            y descriptions at= left,
            x descriptions at=edge bottom,
            % set the `vertical sep' to zero
            horizontal sep=0pt,
            vertical sep=0pt
        },
      width=4.75cm,
      axis y line*=left,
      xlabel={time},
      ylabel={people},
    ]
    \pgfplotsforeachungrouped \p in {1, ..., 20} {
    \edef\tmp{
        \noexpand\nextgroupplot[scaled y ticks=true]
        \noexpand\addplot[only marks,draw opacity=0.5,mark=x,blue] table [x=learned_dist_power, y=learned_dist_turbulence, col sep=comma] {figures/mo_floris/4_turbines/data/dist_\p.csv};
        \noexpand\label{learned_dist_turbulence}
        \noexpand\addplot[only marks,draw opacity=0.5,mark=x,red] table [x=sampled_dist_power, y=sampled_dist_turbulence, col sep=comma] {figures/mo_floris/4_turbines/data/dist_\p.csv};
        \noexpand\label{sampled_dist_turbulence}
       
        }
        \tmp
    }
    \end{groupplot}
    
   
  \end{tikzpicture}
